When Can You Trust Bitcoin? Value-Dependent Block Confirmation to Determine Transaction Finalit

We study financial transaction confirmation finality in Bitcoin as a function of transaction amount and user risk tolerance. A transaction is recorded in a block on a blockchain. However, a transaction may be revoked due to a fork in the blockchain, the odds of which decrease over time but never reach zero. Therefore, a transaction is considered confirmed if its block is sufficiently deep in the blockchain. This depth is usually set empirically at some fixed number such as six blocks. We analyze forks under varying network delays in simulation and actual Bitcoin data. Based on this analysis, we establish a relationship between block depth and the probability of confirmation revocation due to a fork. We use prospect theory to relate transaction confirmation probability to transaction amount and user risk tolerance.

==> reviewerComments.tex <==
======= Review 1 =======

        ------Scores-------
Truly expert in this area of research (1)
Rate the importance and timeliness of the topic 
Acceptable (3)
Quality of presentation
Substantial revision work is needed. (4)
Rate the technical content of the paper, its scientific rigour and novelty.
Questionable work with severe flaws. (5)
Overall evaluation Weak reject (4)

        ------Comments-------
There is no clear indication of the paper’s contribution or how it differentiates itself from prior work and the current state of the art.
- added a text bf statement to make our contribution more clear

The Introduction includes a detailed explanation of block production and forks. This background is fairly standard and might be condensed or omitted in favor of more relevant, novel content.
- seems like we need this and that it can't be shrunk anymore than it is but I did fix some mistakes and reduce our explanation a bit

when talking about making sure if a transaction is confirmed or revoked, what is actually meant by that? Transactions typically remain valid or return to the mempool during reorgs. Unless a double-spending attack is involved, in which case they may be intentionally replaced and then this must be expressed in the paper.
- added a sentence to make this more clear

It’s unclear who the intended beneficiary of this model of this new transaction finality measure is? Is it the receiver that maybe is selling goods? Is it me that is trying to pay someone? This needs to be explained why this is important.
- added to the contribution that this helps vendors, practitioners, and crypto traders

why would a mining pool have any incentive to revoke a transaction? How would they benefit? This needs to be motivated!
while the paper is expressing a need to select a proper waiting time for tx finality, it is never telling us why and for whom it is important?
-added more details to the intro to make it clear why vendors would care about losing money

Applying Prospect Theory is nice, but for someone who doesn't know about this topic the lambda and beta values for the loss function L are very random. This needs to be explained better.
-they aren't random they are given values and accepted by many. made this more clear

It might be useful to introduce Prospect Theory a little more.
- added some more details

LT reflects, and i cite "the user's transaction revocation risk tolerance", but:
The variable c is set, so that LT(1) = 0,5. This choice appears arbitrary, and the transition from discussing risk tolerance to revocation probability is abrupt.
- it was arbitrary but we tried to make it more interesting by saying .5 was easy to understand

How is P rev defined? This needs to be explained here, at this point it is unclear how this value comes to be.
- we calculated it from our simulation and bitcoin data

The evaluation is based solely on simulation. While simulations are useful, there should also be a comparison to real-world behavior.
- we do compare to real world behavior

How likely is a 60-second network delay in the Bitcoin network?
-added a citation that shows 60s is a good worst case as 40s happens often

How frequently do forks occur in practice?
In its current form, the evaluation does not sufficiently reflect actual network conditions and should be better grounded in real-world observations.
-added an old citation from 2013 but it is better than nothing

Given Bitcoin’s 10-minute block time, it seems unlikely that short delays would result in so many chain reorganizations (in this paper called switches). This should be explored in more depth.
-could analyze longer and shorter block times to show the difference in forks but don't have the space for more graphs

The analysis of real Bitcoin data does not seem to support the paper’s novelty. Currently, most wallets treat a depth of six blocks as sufficient for transaction finality. The results presented in the paper reach the same conclusion for a 100 dollar transaction. The paper should explain how this approach provides value beyond simply following the conventional “six blocks” rule.
- we are authenticating the 6 block rule which has value beyond just trusting in conventional wisdom and extends this to the value of the transaction which is different. Made this clearer

======= Review 2 =======

        ------Scores-------
Working in this area of research (2)
Rate the importance and timeliness of the topic 
Good (2)
Quality of presentation Well written. (2)
Rate the technical content of the paper, its scientific rigour and novelty.
Solid work of notable importance. (2)
Overall evaluation Weak accept (2)

        ------Comments-------
I am a little bit disappointed that the authors have not used the allowed 4 pages (for short papers) 
- down to 3 now anyways for a poster

why do the authors not analyze how the results change over time? Instead, only 1000 blocks are taken into account, i.e., blocks from roundabout a week. 
- we obviously don't have time or data to track how the results change over time but that would be cool

It's also disappointing that only 100 miners are taken into account. This limits the usefulness of the results by quite some degree, and at least w.r.t. the number of blocks (or a "window" of blocks), it would have been easy to do further simulation runs.
- we don't have space but agreed

The abstract is quite verbose.
- the abstract was shrunk down

I absolutely DO NOT agree with the claim that the research can also be applied to Ethereum. Most importantly, Ethereum is based on Proof-of-Stake (PoS), which means that the number of forks these days is practically zero. And importantly, before PoS, Ethereum with Proof-of-Work had way more forks than Bitcoin. In Bitcoin, forks are very seldom the case, while in PoW-based Ethereum, they happened every few minutes.
- after digging I agree. Forks in ethereum never last more than a few seconds (since they switched to PoS). Instead we cite Ethereum classic and other bitcoins that use PoW still

Section I: "designed so" => "designed to"
-removed entirely

The information in the references is quite heterogeneous w.r.t. scope and layout. This should be unified.
- overleaf does the references... is there an issue?

======= Review 3 =======

        ------Scores-------
Expertise: Working in this area of research (2)
Relevance to the track and timeliness: 
Good (2)
Quality of presentation
Readable, but revision is needed in some parts. (3)
Technical content and scientific rigour
Valid work but limited contribution. (3)
Overall evaluation: Weak accept (2)

        ------Comments-------
In the introduction, there is a duplicated "However" that should be corrected for clarity.
-fixed

There appears to be a possible inconsistency in the loss function: if β < 0, this would not model diminishing sensitivity as claimed. A more accurate phrasing might be: “the exponent 0 < β < 1 models a diminishing sensitivity to higher losses.”
-fixed

While the paper makes a solid empirical and theoretical case, adding a simple formula or heuristic for practitioners (e.g., how many Bitcoin confirmations are needed based on the transaction amount) would enhance its practical value. While the paper makes a solid empirical and theoretical case, its practical value could be enhanced by offering a simple rule of thumb for practitioners. For example, it could suggest how many confirmations are typically advisable depending on the value of the transaction, giving users a straightforward answer to a common question. Such a heuristic could be informed by both theory and live blockchain data. Since blockchain is observable, an average delay (only for the miners) could be derived or estimated from real conditions. This would ground the paper’s insights in something users can easily apply when deciding how long to wait before considering a transaction final.
- we don't have the space but it seems worth doing. Thoughts?




